Exploring Power Side-Channel Challenges in Embedded Systems Security

Power side-channel (PSC) attacks are widely used in embedded microcontrollers, particularly in cryptographic applications, to extract sensitive information. However, expanding the applications of PSC attacks to broader security contexts in the embedded systems domain faces significant challenges. These include the need for specialized hardware setups to manage high noise levels in real-world targets and assumptions regarding the attacker's knowledge and capabilities. This paper systematically analyzes these challenges and introduces a novel signal-processing method that addresses key limitations, enabling effective PSC attacks in real-world embedded systems without requiring hardware modifications. We validate the proposed approach through experiments on real-world black-box embedded devices, verifying its potential to expand its usage in various embedded systems security applications beyond traditional cryptographic applications.

==> figures/CW_Target.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=3.2cm, angle=0]{figures/STM32F3-Top.png}
    \caption{The ChipWhisperer target board with an integrated shunt resistor on the PCB. This resistor enables accurate measurement of power consumption, which is the current method for conducting precise \psc analysis~\cite{ChipWhispererSTM32Target}.}
    \label{fig:CW_Target}
\end{figure}

==> figures/CovariateShift.tex <==
\begin{figure}
    \centering
    \subfloat[\centering AES128 Instructions]{{\includegraphics[width=4.2cm]{figures/AES128.pdf}}}
    % \qquad
    \subfloat[\centering SHA256 Instructions]{{\includegraphics[width=4.2cm]{figures/SHA256.pdf}}}
    \caption{Different instruction distribution for two cryptography algorithm}
    \label{fig:CovariateShift}
\end{figure}

==> figures/FrequencyResponse.tex <==
\begin{figure}[!h]
    \centering
    \includegraphics[width=7cm]{figures/Frequency_Response.pdf}
    \caption{Frequency response of the high-pass Butterworth filter}
    \label{fig:Freq_Res}
\end{figure}

==> figures/Wavelet_vecs.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=6.4cm]{figures/Wavelet_Vector_Comparison.pdf}
    \caption{Comparison of the extracted fingerprint with our proposed method for two different algorithms.}
    \label{fig:Wavelet_vecs}
\end{figure}

==> sections/ethics.tex <==
\section*{Ethics Considerations and Compliance With the Open Science Policy}

\paragraph{Ethics Considerations}
We are convinced that our paper complies with the high ethical standards of the research community.

None of the experiments discussed in this paper involved participants other than the authors. All hardware used in the experiments is owned by the authors or their institutions and was not shared with other users during the experiments. The crashes we used in our evaluation are collected from publicly accessible resources. 
\paragraph{Compliance With the Open Science Policy}
During the anonymous review process, we provide our code artifact at an anonymous repository~\cite{paper-repo}. We intend to publish the artifact on GitHub once the paper has been accepted.

==> tables/table_applicability.tex <==

\newcommand{\fullcircle}{\tikz\draw[fill=black] (0,0) circle (.5ex);}
\newcommand{\halfcircle}{
    \begin{tikzpicture}
    \draw (0,0) circle (.5ex);
    \fill[black] (0,-.5ex) arc[start angle=-90,end angle=90,radius=.5ex];
    \end{tikzpicture}
}
\newcommand{\mincircle}{
    \begin{tikzpicture}
    \draw (0,0) circle (.5ex);
    \fill[black] (0,0) -- (0ex,0.5ex) arc[start angle=90,end angle=180,radius=.5ex] -- cycle;
    \end{tikzpicture}
}
\newcommand{\nullcircle}{\tikz\draw (0,0) circle (.5ex);}

\begin{table*}[!h]
    \centering
\begin{tabular}{|l|l|l|c|c|c|c|c|} 
\hline
Data Fidelity                        & ISA                     & Firmware       & Disassembly & Fuzzing & SCA & External Bus Activity & IDS  \\ 
\hline
\multirow{3}{*}{Ops/Opr  }      & \multirow{2}{*}{Known } & Avail.     & N/A                          & \fullcircle{} (GB)  & N/A                           & N/A         & \fullcircle{} (WB)                             \\ 
\cline{3-8}
                                &                         & N/A & \fullcircle                  & \fullcircle{} (BB)  & \halfcircle{} (BB)                   & \fullcircle{} (BB)              & \halfcircle{} (GB?)                  \\ 
\cline{2-8}
                                & \multicolumn{2}{c|}{Unknown}             & \mincircle                   & \fullcircle{} (BB)  & \halfcircle{} (BB)                   & \fullcircle{} (BB)        & \halfcircle{} (BB)                        \\ 
\hline
\multirow{3}{*}{Basic Blocks  } & \multirow{2}{*}{Known}  & Avail.     & N/A                          & \fullcircle{} (GB)  & N/A                           & N/A               & \fullcircle                         \\ 
\cline{3-8}
                                &                         & N/A & \mincircle                   & \fullcircle{} (BB)  & \halfcircle{} (BB)                   & \fullcircle{} (BB)                 & \halfcircle               \\ 
\cline{2-8}
                                & \multicolumn{2}{c|}{Unknown}             & \nullcircle                  & \fullcircle{} (BB)  & \halfcircle{} (BB)                    & \fullcircle{} (BB)            & \halfcircle                    \\ 
\hline
\multirow{3}{*}{Power trace  }  & \multirow{2}{*}{Known~} & Avail.     & N/A                          & \halfcircle{} (GB)  & N/A                           & N/A               & \mincircle                        \\ 
\cline{3-8}
                                &                         & N/A & \nullcircle                  & \halfcircle{} (BB)  & \mincircle{} (BB)                     & \fullcircle{} (BB)                & \mincircle                \\ 
\cline{2-8}
                                & \multicolumn{2}{c|}{Unknown}             & \nullcircle                  & \halfcircle{} (BB)  & \mincircle{} (BB)                     & \fullcircle{} (BB)             & \mincircle                   \\
\hline
\end{tabular}
    \caption{\ulysse{ find caption}}
    \label{tab:applicability}
\end{table*}
